Language Agnostic Code Embeddings

Recently, code language models have achieved notable advancements in addressing a diverse array of essential code comprehension and generation tasks. Yet, the field lacks a comprehensive deep dive and understanding of the code embeddings of multilingual code models. In this paper, we present a comprehensive study on multilingual code embeddings, focusing on the cross-lingual capabilities of these embeddings across different programming languages. Through probing experiments, we demonstrate that code embeddings comprise two distinct components: one deeply tied to the nuances and syntax of a specific language, and the other remaining agnostic to these details, primarily focusing on semantics. Further, we show that when we isolate and eliminate this language-specific component, we witness significant improvements in downstream code retrieval tasks, leading to an absolute increase of up to +17 in the Mean Reciprocal Rank (MRR).

==> plots/lang_dist/lang_distance.tex <==

\begin{figure*}[t]
  \centering

  \begin{subfigure}[b]{0.19\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/lang_dist/language_distance_codebert.pdf}
    \subcaption{CodeBERT}
    \label{fig:language_distance_codebert}
  \end{subfigure}
  \begin{subfigure}[b]{0.19\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/lang_dist/language_distance_graphcodebert.pdf}
    \subcaption{GraphCodeBERT}
    \label{fig:language_distance_graphcodebert}
  \end{subfigure}
  \begin{subfigure}[b]{0.19\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/lang_dist/language_distance_unixcoder.pdf}
    \subcaption{UnixCoder}
    \label{fig:language_distance_unixcoder}
  \end{subfigure}
  \begin{subfigure}[b]{0.19\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/lang_dist/language_distance_starencoder.pdf}
    \subcaption{StarEncoder}
    \label{fig:language_distance_starencoder}
  \end{subfigure}
  \begin{subfigure}[b]{0.19\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/lang_dist/language_distance_codet5+.pdf}
    \subcaption{CodeT5+}
    \label{fig:language_distance_codet5+}
  \end{subfigure}\\[0.16in] 
  \begin{subfigure}[b]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/heatmaps/original_heatmap.pdf}
    \subcaption{Original}
    \label{fig:original_distance_heatmap}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/heatmaps/centering_heatmap.pdf}
    \subcaption{Centering}
    \label{fig:centering_distance_heatmap}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/heatmaps/lrd_heatmap.pdf}
    \subcaption{LRD}
    \label{fig:lrd_distance_heatmap}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{plots/heatmaps/cs-lrd_heatmap.pdf}
    \subcaption{CS-LRD}
    \label{fig:cs-lrd_distance_heatmap}
  \end{subfigure}
  \caption{Figures \ref{fig:language_distance_codebert} to \ref{fig:language_distance_codet5+} shows distance beween langauge geometric medians before and after removing language component . }
  \label{fig:language_distance}
\end{figure*}
